Rubric-CEPR: Self-Evolving Image Editing via Reward-Verified Self-Distillation

Instruction-guided image editors have become highly capable, yet improving them further still depends on human-edited training pairs or external reward models. Such supervision is costly to obtain and can reward plausible failures: a realistic output may leave the requested change undone or alter content that should be preserved. In this work, we strive to improve a pretrained image editor using only its own generations, without human-edited targets or an external training-time reward model. To this end, we propose a self-evolving framework, named Rubric-CEPR, that verifies the editor's own samples with its internal representations through a rubric-augmented Contrastive Edit-Preservation Reward (CEPR). A Planner proposes structured edit instructions from unlabeled images, the Editor samples multiple candidate edits, and a frozen Critic scores each candidate with decomposed rubric checks for edit realization, removal of the old state, and content preservation, using features already exposed by the editor. Non-compensatory gates reject infeasible candidates, and the best verified candidate is distilled into the editor through lightweight adapter training. On Qwen-Image-Edit, Rubric-CEPR improves ImgEdit from 4.36 to 4.60 (+5.5%), with a +24.9% gain on object isolation, and transfers to GEdit-Bench and Complex-Edit. The same procedure also improves Step1X-Edit by +7.8% on ImgEdit. We hope our approach will serve as a solid baseline for image editors that improve themselves from their own verified samples. Our code is publicly available at https://github.com/riteshthawkar/Rubric-CEPR

==> figures/teaser_tikz.tex <==
% Teaser figure drawn natively in TikZ (vector, paper fonts).
% Five stages: (1) Planner proposes, (2) Editor samples K candidates, (3) frozen Critic
% scores them, (4) best-of-K selection, (5) distillation into the next-round adapters.
% Designed at 14 cm wide and shown at 0.95\linewidth (Figure 1 must stay on page 1).
% Needs: tikz, amsmath, and the TikZ libraries arrows.meta, calc.
\begingroup
\definecolor{tkPlanner}{RGB}{201,103,4}
\definecolor{tkEditor}{RGB}{16,133,72}
\definecolor{tkCritic}{RGB}{0,87,184}
\definecolor{tkInk}{RGB}{21,62,117}
\definecolor{tkRed}{RGB}{184,56,56}
\definecolor{tkBlue}{RGB}{47,102,196}
\definecolor{tkLeaf}{RGB}{74,146,84}
\tikzset{
  tkbox/.style={draw=#1!78!black, fill=#1!8, rounded corners=3pt, line width=0.7pt,
                align=center, inner sep=3pt, font=\footnotesize},
  tkgray/.style={draw=black!50, fill=black!3.5, rounded corners=3pt, line width=0.7pt,
                 align=center, inner sep=3pt, font=\footnotesize},
  tkplain/.style={draw=black!55, fill=white, rounded corners=3pt, line width=0.7pt,
                  align=left, inner sep=3pt, font=\scriptsize},
  tkarrow/.style={-{Stealth[length=5pt,width=4.2pt]}, line width=0.9pt, draw=black!75},
  tkdash/.style={-{Stealth[length=5pt,width=4.2pt]}, line width=0.9pt,
                 dash pattern=on 3.2pt off 2.2pt, draw=tkInk!85, rounded corners=3pt},
  tklabel/.style={font=\scriptsize, align=center, inner sep=1.5pt},
}
% Scene on a unit square: cube colour (#1), ball colour (#2), plant present (#3 = 1 or 0).
\newcommand{\tkscene}[3]{%
  \shade[top color=white, bottom color=black!9] (0,0.27) rectangle (1,1);
  \fill[black!13] (0,0) rectangle (1,0.27);
  \fill[black!22] (0.42,0.17) ellipse (0.31 and 0.045);
  \fill[#1!82!black] (0.16,0.19) rectangle (0.50,0.53);
  \fill[#1!45!white] (0.16,0.53) -- (0.26,0.63) -- (0.60,0.63) -- (0.50,0.53) -- cycle;
  \fill[#1!62!black] (0.50,0.19) -- (0.60,0.29) -- (0.60,0.63) -- (0.50,0.53) -- cycle;
  \fill[#2!90!black] (0.38,0.76) circle (0.125);
  \fill[#2] (0.375,0.765) circle (0.108);
  \fill[white,opacity=0.65] (0.335,0.805) circle (0.035);
  \ifnum#3=1
    \fill[black!20] (0.81,0.18) ellipse (0.13 and 0.03);
    \fill[brown!65!black] (0.72,0.19) -- (0.90,0.19) -- (0.87,0.36) -- (0.75,0.36) -- cycle;
    \begin{scope}[shift={(0.81,0.36)}]
      \fill[tkLeaf] [rotate=-35] (0,0.12) ellipse (0.035 and 0.13);
      \fill[tkLeaf!85!black] (0,0.14) ellipse (0.035 and 0.15);
      \fill[tkLeaf] [rotate=35] (0,0.12) ellipse (0.035 and 0.13);
    \end{scope}
  \fi
  \draw[black!50, line width=0.4pt] (0,0) rectangle (1,1);
}
% Pass / reject badges centred at #1.
\newcommand{\tkcheck}[1]{\begin{scope}[shift={#1}]
  \fill[tkEditor] (0,0) circle (0.17);
  \draw[white, line width=1pt, line cap=round, line join=round]
    (-0.085,0.0) -- (-0.025,-0.07) -- (0.095,0.075);\end{scope}}
\newcommand{\tkcross}[1]{\begin{scope}[shift={#1}]
  \fill[tkRed] (0,0) circle (0.17);
  \draw[white, line width=1pt, line cap=round]
    (-0.07,-0.07) -- (0.07,0.07) (-0.07,0.07) -- (0.07,-0.07);\end{scope}}
% Stage number tag centred at #1.
\newcommand{\tknum}[2]{\node[circle, fill=tkInk, text=white, inner sep=0pt, minimum size=0.36cm,
  font=\scriptsize\bfseries] at #1 {#2};}
% Robot head icon centred at origin (about 0.62 x 0.62 cm); #1 = accent colour.
\newcommand{\tkrobot}[1]{%
  \draw[#1!80!black, line width=0.6pt] (0,0.26) -- (0,0.36); \fill[#1!80!black] (0,0.375) circle (0.035);
  \fill[#1!70!white, draw=#1!80!black, line width=0.5pt] (-0.30,-0.02) rectangle (-0.24,0.12);
  \fill[#1!70!white, draw=#1!80!black, line width=0.5pt] (0.24,-0.02) rectangle (0.30,0.12);
  \fill[#1!8!white, draw=black!60, line width=0.6pt, rounded corners=2.5pt] (-0.24,-0.24) rectangle (0.24,0.26);
  \fill[tkBlue!30!white, draw=black!45, line width=0.4pt, rounded corners=1.5pt] (-0.18,-0.14) rectangle (0.18,0.17);
  \fill[tkInk] (-0.075,0.06) circle (0.032); \fill[tkInk] (0.075,0.06) circle (0.032);
  \draw[tkInk, line width=0.4pt, line cap=round] (-0.07,-0.04) .. controls (-0.03,-0.085) and (0.03,-0.085) .. (0.07,-0.04);}
% Clipboard icon centred at origin (about 0.4 x 0.58 cm); #1 = accent colour.
\newcommand{\tkclip}[1]{%
  \fill[#1!55!white, draw=#1!80!black, line width=0.5pt, rounded corners=1.5pt] (-0.20,-0.28) rectangle (0.20,0.26);
  \fill[white, draw=black!35, line width=0.3pt] (-0.145,-0.22) rectangle (0.145,0.18);
  \fill[black!65, rounded corners=0.8pt] (-0.08,0.20) rectangle (0.08,0.32);
  \draw[black!50, line width=0.4pt, line cap=round]
    (-0.09,0.08) -- (0.09,0.08) (-0.09,-0.02) -- (0.09,-0.02) (-0.09,-0.12) -- (0.03,-0.12);}
% Layered-features icon centred at origin.
\newcommand{\tklayers}{%
  \foreach \y/\a in {-0.17/42, -0.02/28, 0.13/14}{
    \fill[tkCritic!\a!white, draw=tkCritic!80!black, line width=0.5pt, line join=round]
      (-0.2,\y) -- (0.14,\y) -- (0.24,\y+0.11) -- (-0.1,\y+0.11) -- cycle;}}
% Shield-with-check icon centred at origin.
\newcommand{\tkshield}{%
  \fill[tkCritic!14, draw=tkCritic!80!black, line width=0.6pt, line join=round]
    (-0.2,0.24) -- (0.2,0.24) -- (0.2,0.02) .. controls (0.2,-0.14) and (0.08,-0.22) .. (0,-0.28)
    .. controls (-0.08,-0.22) and (-0.2,-0.14) .. (-0.2,0.02) -- cycle;
  \draw[tkEditor, line width=1.1pt, line cap=round, line join=round]
    (-0.09,0.0) -- (-0.02,-0.08) -- (0.1,0.1);}
%
\resizebox{0.95\linewidth}{!}{%
\begin{tikzpicture}[x=1cm,y=1cm]
  % =============== row 1: propose and edit ===============
  % (1) unlabeled source images, stacked
  \begin{scope}[shift={(0.40,5.35)}, scale=1.15] \tkscene{tkBlue}{tkLeaf}{1} \end{scope}
  \begin{scope}[shift={(0.25,5.20)}, scale=1.15] \tkscene{tkLeaf}{tkRed}{0} \end{scope}
  \begin{scope}[shift={(0.10,5.05)}, scale=1.15] \tkscene{tkRed}{tkRed}{1} \end{scope}
  \node[tklabel] at (0.82,4.58) {unlabeled\\images $x$};
  % Planner
  \node[tkbox=tkPlanner, minimum width=1.75cm, minimum height=2.3cm] (planner) at (2.95,5.875) {};
  \begin{scope}[shift={(2.95,6.38)}, scale=1.6] \tkrobot{tkPlanner} \end{scope}
  \node[font=\footnotesize, align=center] at (2.95,5.18) {\textbf{\emph{Planner}}\\[-1pt]\scriptsize LoRA, $P_\psi$};
  \tknum{(2.08,6.98)}{1}
  % structured proposal card
  \node[tkplain, text width=3.25cm, anchor=west, minimum height=2.3cm] (spec) at (4.2,5.875)
    {\textbf{Structured proposal}\\[2pt]
     $c$: ``Make the ball blue''\\[1pt]
     $s$: edit type, entities, region,\\
     \phantom{$s$: }required / forbidden state,\\
     \phantom{$s$: }content to preserve};
  \begin{scope}[shift={(7.12,6.62)}, scale=0.95] \tkclip{tkPlanner} \end{scope}
  % Editor
  \node[tkbox=tkEditor, minimum width=1.75cm, minimum height=2.3cm] (editor) at (9.0,5.875) {};
  \begin{scope}[shift={(9.0,6.38)}, scale=1.6] \tkrobot{tkEditor} \end{scope}
  \node[font=\footnotesize, align=center] at (9.0,5.18) {\textbf{\emph{Editor}}\\[-1pt]\scriptsize LoRA, $E_\theta$};
  \tknum{(8.13,6.98)}{2}
  \draw[tkarrow] (1.68,5.875) -- (planner.west);
  \draw[tkarrow] (planner.east) -- (spec.west);
  \draw[tkarrow] (spec.east) -- (editor.west);
  \draw[tkarrow] (editor.east) -- (10.3,5.875);
  % K candidate edits (2 x 2)
  \begin{scope}[shift={(10.4,5.95)}, scale=1.45]  \tkscene{tkRed}{tkBlue}{1} \end{scope}
  \begin{scope}[shift={(12.0,5.95)}, scale=1.45]  \tkscene{tkRed}{tkRed}{1} \end{scope}
  \begin{scope}[shift={(10.4,4.35)}, scale=1.45]  \tkscene{tkBlue}{tkBlue}{1} \end{scope}
  \begin{scope}[shift={(12.0,4.35)}, scale=1.45]  \tkscene{tkRed}{tkBlue}{0} \end{scope}
  \node[tklabel] at (11.925,7.65) {$K$ candidate edits $\{y_i\}$};
  % =============== row 2: verify, select, distill ===============
  % (3) frozen Critic
  \node[tkbox=tkCritic, minimum width=6.75cm, minimum height=3.3cm, anchor=south west]
    (critic) at (7.2,0.25) {};
  \begin{scope}[shift={(7.62,3.27)}, scale=0.62] \tkrobot{tkCritic} \end{scope}
  \node[font=\footnotesize, anchor=west, inner sep=0pt] at (7.92,3.27)
    {\textbf{\emph{Critic}} \scriptsize(frozen)};
  \tknum{(7.2,3.55)}{3}
  \foreach \cx/\ttl/\txt in {
    8.375/{Features}/{Qwen-VL\\ support, gain,\\ VAE latents},
    10.575/{Rubric checks}/{edit realization\\ old-state removal\\ preservation\\ validity},
    12.775/{Gates}/{every applicable\\ check must pass,\\ else $G{=}0$}}{
    \node[tkplain, minimum width=1.95cm, minimum height=2.2cm, anchor=south] at (\cx,0.78) {};
    \node[tklabel, text width=1.8cm, anchor=north] at (\cx,2.28) {\textbf{\ttl}\\[1pt]\txt};}
  \begin{scope}[shift={(8.375,2.62)}, scale=0.95] \tklayers \end{scope}
  \begin{scope}[shift={(10.575,2.62)}, scale=0.95] \tkclip{tkCritic} \end{scope}
  \begin{scope}[shift={(12.775,2.62)}, scale=0.95] \tkshield \end{scope}
  \draw[tkarrow] (9.35,1.9) -- (9.60,1.9);
  \draw[tkarrow] (11.55,1.9) -- (11.80,1.9);
  \node[font=\footnotesize, inner sep=1pt] at (10.575,0.50) {$R = G\cdot\sqrt{E\times P}$};
  \draw[tkarrow] (11.925,4.28) -- node[tklabel, right, xshift=1pt] {score} (11.925,3.57);
  % (4) best-of-K selection
  \node[tkgray, minimum width=2.85cm, minimum height=3.15cm, anchor=south west]
    (select) at (3.8,0.25) {};
  \node[tklabel] at (5.225,3.17) {\textbf{Best-of-$K$} selection};
  \begin{scope}[shift={(3.95,1.22)}, scale=1.1] \tkscene{tkRed}{tkBlue}{1} \end{scope}
  \begin{scope}[shift={(5.40,1.22)}, scale=1.1] \tkscene{tkRed}{tkRed}{1} \end{scope}
  \tkcheck{(4.50,2.66)}
  \tkcross{(5.95,2.66)}
  \node[tklabel, text=tkEditor!85!black] at (4.50,0.82) {selected $y^\star$};
  \node[tklabel, text=tkRed] at (5.95,0.82) {rejected};
  \tknum{(3.8,3.4)}{4}
  \draw[tkarrow] (7.2,1.9) -- (6.65,1.9);
  % (5) next-round adapters
  \node[tkgray, minimum width=3.25cm, minimum height=3.15cm, anchor=south west]
    (next) at (0.05,0.25) {};
  \node[font=\scriptsize, inner sep=0pt] at (1.675,0.52) {\textbf{Next round} $(t\!+\!1)$};
  \node[tkbox=tkPlanner, minimum width=1.45cm, minimum height=2.0cm] (p2) at (0.9,1.85) {};
  \begin{scope}[shift={(0.9,2.28)}, scale=1.15] \tkrobot{tkPlanner} \end{scope}
  \node[font=\footnotesize, align=center] at (0.9,1.28) {\emph{Planner}\\[-1pt]\scriptsize $P_{t+1}$};
  \node[tkbox=tkEditor, minimum width=1.45cm, minimum height=2.0cm] (e2) at (2.45,1.85) {};
  \begin{scope}[shift={(2.45,2.28)}, scale=1.15] \tkrobot{tkEditor} \end{scope}
  \node[font=\footnotesize, align=center] at (2.45,1.28) {\emph{Editor}\\[-1pt]\scriptsize $E_{t+1}$};
  \tknum{(0.05,3.4)}{5}
  \draw[tkarrow] (3.8,1.9) -- (3.3,1.9);
  % parameter updates fed back to the next round (dashed)
  \draw[tkdash] (p2.north) -- ++(0,1.4) -| (planner.south);
  \node[tklabel, fill=white] at (1.92,4.25) {proposal SFT};
  \draw[tkdash] (e2.north) -- ++(0,1.1) -| (editor.south);
  \node[tklabel, fill=white] at (5.7,3.95) {weighted denoising SFT};
\end{tikzpicture}}
\endgroup

